A hierarchical Bayesian perspective on majorization-minimization for non-convex sparse regression: application to M/EEG source imaging

Majorization-minimization (MM) is a standard iterative optimization technique which consists in minimizing a sequence of convex surrogate functionals. MM approaches have been particularly successful to tackle inverse problems and statistical machine learning problems where the regularization term is a sparsity-promoting concave function. However, due to non-convexity, the solution found by MM depends on its initialization. Uniform initialization is the most natural and often employed strategy as it boils down to penalizing all coefficients equally in the first MM iteration. Yet, this arbitrary choice can lead to unsatisfactory results in severely under-determined inverse problems such as source imaging with magneto- and electro-encephalography (M/EEG). The framework of hierarchical Bayesian modeling (HBM) is an alternative approach to encode sparsity. This work shows that for certain hierarchical models, a simple alternating scheme to compute fully Bayesian maximum a posteriori (MAP) estimates leads to the exact same sequence of updates as a standard MM strategy (cf. the Adaptive Lasso). With this parallel outlined, we show how to improve upon these MM techniques by probing the multimodal posterior density using Markov Chain Monte-Carlo (MCMC) techniques. Firstly, we show that these samples can provide well-informed initializations that help MM schemes to reach better local minima. Secondly, we demonstrate how it can reveal the different modes of the posterior distribution in order to explore and quantify the inherent uncertainty and ambiguity of such ill-posed inference procedure. In the context of M/EEG, each mode corresponds to a plausible configuration of neural sources, which is crucial for data interpretation, especially in clinical contexts. Results on both simulations and real datasets show how the number or the type of sensors affect the uncertainties on the estimates.

==> sections/experiments.tex <==
%!TEX root = ../LpHypermodelsEMEG.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{First Results}
\label{sec:first_results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\paragraph{Setting}

The head model is a quite realistic, anisotropic FEM model and the sensors are an artificial MEG cap consisting of just 63 sensors, but that is not too important here.
No noise added but we assumed an SNR of 20dB.
\Cref{fig:RefSol} shows the reference sources and \Cref{fig:TwoDipScan} a two-dipole scan applied to the data to show that there is no uniqueness issue with this source configuration:
The references sources can be recovered with the strong a priori knowledge that there are 2 of them.


\begin{figure}[tb]
\centering
\subfloat[][XY view]
{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_RefSol_XY}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_RefSol_XZ}}
\hfill
\caption{Reference sources to recover (green cones). \label{fig:RefSol}}
\end{figure}


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_TwoDipScan_XY}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_TwoDipScan_XZ}}
\hfill
\caption{A two-dipole scan (red cones) applied to the data to show that the references sources (green cones) can be recovered from the data. \label{fig:TwoDipScan}}
\end{figure}


\paragraph{MNE}

We first compute the minimum norm estimate, \ie $\ell_{2,2}$-regularized, see \Cref{fig:MNE}.
The parameter $\lambda$ is found via the discrepancy principle (demand that $\fronormsq{\bfG \hat{\bfX} - \bfM} = \sigma^2 m$ \jo{$m$ is this now $n d$?} up to a tolerance) which leads to a relative residuum $\fronorm{\bfG \hat{\bfX} - \bfM}/\fronorm{\bfX}$) of 0.224.
As we see, it fails to separate the two sources.

\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_MNE_XY}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_MNE_XZ}}
\hfill
\caption{MNE (red cones) and references sources (green cones). Relative residuum = 0.224. \label{fig:MNE}}
\end{figure}


\paragraph{sLORETA}

Next we compute the sLORETA result, based upon the $\lambda$ of the MNE, see \Cref{fig:sLORETA}.  It also fails to separate the two sources.

\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_sLORETA_XY}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_sLORETA_XZ}}
\hfill
\caption{sLORETA (red spheres) and references sources (green cones).
\label{fig:sLORETA}}
\end{figure}


\paragraph{MCE ($\ell_{2,1}$}

The minimum current estimate (MCE), \ie $\ell_{2,1}$-regularized, is shown in \Cref{fig:MCE}. $\lambda$ is found via the discrepancy principle but with more tolerance compared to MNE which leads to a relative residuum $\fronorm{\bfG \hat{\bfX} - \bfM}/\fronorm{\bfX}$) of 0.208. The zoom-in shows that it finds three visible sources, not a great result, which is why I chose this source configuration, if the MCE would already do a good job, using the more sophisticated methods would somehow be pointless.

\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21_XY}}
\hfill
\subfloat[][XY view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21_XZ}}
\caption{$\ell_{2,1}$ regularized solution (red cones) and references sources (green cones). Relative residuum = 0.208. \label{fig:MCE}}
\end{figure}


\paragraph{iteratively re-weighted $\ell_{2,1}$}

Next we compute iteratively re-weighted $\ell_{2,1}$ solutions which corresponds to computing a full-MAP estimate by an alternating optimization using a standard gamma hyperprior (\lcf \Cref{subsec:L21withGamma}).
First, we start with a uniform $\gamma$ as a starting value, \ie the first iteration the MCE computed in the last paragraph.
The result is shown in \Cref{fig:iL21uni}, the relative residuum is 0.122 (shown is the result after 10 iterations, but after 5 iterations, the resuls did not really change anymore).
The support of the initial MCE solution did not change anymore, just the orientation and amplitude of the sources changed slightly.
Then, we used an sLORETA inspired weighing as the first weighting, the result is shown in \Cref{fig:iL21sLORETA}, the relative residuum is 0.084, but the result is not really much better.


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_iL21uni_XY}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_iL21uni_XZ}}
\caption{iteratively re-weighted $\ell_{2,1}$ solution, uniform start weighting (red cones) and references sources (green cones). Relative residuum = 0.122. \label{fig:iL21uni}}
\end{figure}

\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_iL21sL_XY}}
\hfill
\subfloat[][XZ view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_iL21sL_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_iL21sL_XZ}}
\caption{iteratively re-weighted $\ell_{2,1}$ solution, sLORETA-based start weighting (red cones) and references sources (green cones). Relative residuum = 0.084.
\label{fig:iL21sLORETA}}
\end{figure}


\paragraph{Bregman iterations applied to $\ell_{2,1}$}

I did not discuss this above, but if the problem is just to get rid of the amplitude bias introduced by the $\ell_{2,1}$ regularizations, another thing one can do it to use Bregman iterations, in which one also has to solve a sequence of $\ell_{2,1}$-regularized problems, but the $\lambda$ stays the same while the data changes. In principle, once a source location is active, it is not regularized any more. The whole iteration converges to the solution of
\begin{equation}
\argmin_u \sum_i^n \norm{u_{[i]}}_2^1 \qquad such \;\; that \qquad A u = f
\end{equation}
but has some nice features. I stopped the scheme after 50 iterations, which leads to a relative residuum of 0.016 and \Cref{fig:Breg}. It looks a little better than the other solutions, but not yet what we want.


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_BregL21_XY}}
\hfill
\subfloat[][XZ view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_BregL21_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_BregL21_XZ}}
\caption{Bregman iterations on $\ell_{2,1}$ regularization, iter 50 (red cones) and references sources (green cones). Relative residuum = 0.016. \label{fig:Breg}}
\end{figure}



\paragraph{CM estimate for $\ell_{2,1}$ prior}

While the MCE is the MAP estimate for using an $\ell_{2,1}$ prior, we now start to use MCMC to compute the corresponding CM estimate.
It has a slightly lower relative residual with 0.175 compared to the MCE, but the solution is not sparse any more (although sparser than the MNE, \lcf \Cref{fig:L21CM}


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21_CM_XY}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21_CM_XZ}}
\caption{CM estimate for $\ell_{2,1}$ prior (red cones) and references sources (green cones). Relative residuum = 0.175.
\label{fig:L21CM}}
\end{figure}



\paragraph{$\ell_{2,2}$ Hypermodel with Inverse Gamma (\lcf Section \ref{subsec:L22withInvGamma})}

Now we turn to the hypermodels and start with the compuationally most easy one, the $\ell_{2,2}$ model with inverse gamma hyperprior.
I chose $\alpha = 0.5$, $\beta = 5 \cdot 10^{-5}$ based on the results of my thesis and ran a long MCMC-chain.
The CM estimate $\xCM$ has a residual of 0.024 and is shown in \Cref{fig:L22InvGamCMall}.
One can see that it finds a cloud of small dipoles around the second dipole, but the result is not convincing either.
If one uses the corresponding $\gamCM$ to initialize the alternating optimization to compute a MAP estimate, we obtain \Cref{fig:L22InvGamMAPall}, a solution which completely misses the left dipole, with relative residuum of 0.314.


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L2iGam_CM_all_XY}}
\hfill
\subfloat[][XZ view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L2iGam_CM_all_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L2iGam_CM_all_XZ}}
\caption{CM estimate for $\ell_{2,2}$ hypermodel with inverse gamma hyperprior (red cones) and references sources (green cones).
Relative residuum = 0.024.
\label{fig:L22InvGamCMall}}
\end{figure}


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1iGam_MAP_CMall_XY}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1iGam_MAP_CMall_XZ}}
\caption{MAP estimate for $\ell_{2,2}$ hypermodel with inverse gamma hyperprior, initialized at the CM estimate based on the whole MCMC chain (red cones) and references sources (green cones).
Relative residuum = 0.314.
\label{fig:L22InvGamMAPall}}
\end{figure}


\paragraph{$\ell_{2,1}$ Hypermodel with Inverse Gamma (\lcf Section \ref{subsec:L21withInvGamma})}

As a direct comparison, we change $p$ from $2$ to $1$ (and use $\alpha = 0.5$, $\beta = 10^-4$). Figures \ref{fig:L21InvGamCMall} and \ref{fig:L21InvGamMAPall} show the results, which look rather similar and have similar relative residuals.


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1iGam_CM_all_XY}}
\hfill
\subfloat[][XZ view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1iGam_CM_all_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1iGam_CM_all_XZ}}
\caption{CM estimate for $\ell_{2,1}$ hypermodel with inverse gamma hyperprior (red cones) and references sources (green cones).
Relative residuum = 0.034.
\label{fig:L21InvGamCMall}}
\end{figure}

\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1iGam_MAP_CMall_XY}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1iGam_MAP_CMall_XZ}}
\caption{MAP estimate for $\ell_{2,1}$ hypermodel with inverse gamma hyperprior, initialized at the CM estimate based on the whole MCMC chain (red cones) and references sources (green cones).
Relative residuum = 0.302.\label{fig:L21InvGamMAPall}}
\end{figure}


\paragraph{$\ell_{2,1}$ Hypermodel with Gamma (\lcf \Cref{subsec:L21withGamma})}

Now this again corresponds to the model behind the iteratively re-weighted $\ell_{2,1}$ approach, as we chose $\alpha = d+1 = 4$ and we set $\beta = 4/\lambda^2$, where $\lambda$ is the one of the MCE solution.
The results are sown in Figures \ref{fig:L21GamCMall}, \ref{fig:L21GamMAPall} and relative residual of the CM estimate is 0.105 and of the MAP estimate 0.146.
The results haven't really improved over those obtained from uniform or sLORETA based initialization.


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1Gam_CM_all_XY}}
\hfill
\subfloat[][XZ view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1Gam_CM_all_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1Gam_CM_all_XZ}}
\caption{CM estimate for $\ell_{2,1}$ hypermodel with gamma hyperprior (red cones) and references sources (green cones).
Relative residuum = 0.105.
\label{fig:L21GamCMall}}
\end{figure}


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1Gam_MAP_CMall_XY}}
\hfill
\subfloat[][XY view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1Gam_MAP_CMall_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_HBM_L1Gam_MAP_CMall_XZ}}
\caption{MAP estimate for $\ell_{2,1}$ hypermodel with gamma hyperprior, initialized at the CM estimate based on the whole MCMC chain (red cones) and references sources (green cones).
Relative residuum = 0.146.
\label{fig:L21GamMAPall}}
\end{figure}

\clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Second Results}
\label{sec:second_restults}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


After these first results were not too encouraging, I had a closer look at the MCMC chains.
In \Cref{fig:U5chains}, I plotted the amplitudes of the 5 strongest sources as they change over the chain.
For the $\ell_{2,2}$ model, one source is always on (probably the one on the right in \Cref{fig:L22InvGamCMall}, while different sources are switched on and off with about half the amplitude of the blue one (they build the cluster of sources on the left in \Cref{fig:L22InvGamCMall}).
This tell us that most of the probable solutions that the hypermodel finds consist of the one right source being active together with one source on the left.
For the $\ell_{2,1}$ model with the inverse gamma hyperprior, the situation looks different, the samplers seems to jump between different combinations of sources more frequently.
This is what I had hoped for, so some reasons to be optimistic here. The $\ell_{2,1}$ model with the gamma hyperprior looks a bit different, one source is on for most of the time and all others are significantly smaller.
I might have to rerun this part with different parameter settings.

If one picks out parts of the chain that look interesting in this picture and takes some value for $\gamma$ at these locations as an initialization for the alternating optimization to compute the MAP estimate, one can find local optima that give quite nice results.
To make this more systematic, I did it for every sample in the chains, and plotted the relative residuals of the local MAP estimates in \Cref{fig:RelResChains}.
One can see that the MAP estimates initialized in this way can reach far lower relative residuals compared to all MAP estimates presented in the last section, which could indicate that the initialization with the CM estimate is rather sub-optimal and that far better results could be obtained.
One can also see that the samplers stay in the attractor of a mode for quite a while, see \Cref{fig:RelResChainsZoom}.
Figures \ref{fig:L22InvGamMAPbRR}-\ref{fig:L21GamMAPbRR} show the MAP estimates that obtained the best relative residuals. They all look way better (the result with the $\ell_{2,1}$ model with the gamma hyperprior might suffer from a bad parameterization, I will re-run this bit), which means that there is hope! I'll have to look into the topic more closely and run some more tests.


\begin{figure}[tb]
\centering
\subfloat[][$\ell_{2,2}$ with inverse gamma hyperprior]{\includegraphics[width=.8\textwidth]{LpHyperModelsMEG_s12_HBM_L2iGam_traceU5}}\\
\subfloat[][$\ell_{2,1}$ with inverse gamma hyperprior]{\includegraphics[width=.8\textwidth]{LpHyperModelsMEG_s12_HBM_L1iGam_traceU5}}\\
\subfloat[][$\ell_{2,1}$ with gamma hyperprior]{\includegraphics[width=.8\textwidth]{LpHyperModelsMEG_s12_HBM_L1Gam_traceU5}}
\caption{The amplitudes of the 5 locations with the largest overall amplitudes are shown as a function of MCMC sample $k$.
\label{fig:U5chains}}
\end{figure}




\begin{figure}[tb]
\centering
\subfloat[][$\ell_{2,2}$ with inverse gamma hyperprior ($SSR = 100$!!!)]{\includegraphics[width=.7\textwidth]{RelResLocalModesL2InvGam}}\\
\subfloat[][$\ell_{2,1}$ with inverse gamma hyperprior ($SSR = 1$)]{\includegraphics[width=.7\textwidth]{RelResLocalModesL1InvGam}}\\
\subfloat[][$\ell_{2,1}$ with gamma hyperprior ($SSR = 1$)]{\includegraphics[width=.7\textwidth]{RelResLocalModesL1Gam}}
\caption{The relative residual of MAP estimates computed by the alternating optimization initialized at $\gamma_k$ is shown as a function of MCMC sample $k$.
Note that the chains were run with very different sub-sampling factors ($SSR$), so a direct comparison of performance and mixing is not possible.
\label{fig:RelResChains}}
\end{figure}


\begin{figure}[tb]
\centering
\subfloat[][$\ell_{2,2}$ with inverse gamma hyperprior ($SSR = 100$!!!)]{\includegraphics[width=.7\textwidth]{RelResLocalModesL2InvGamZoom}}\\
\subfloat[][$\ell_{2,1}$ with inverse gamma hyperprior ($SSR = 1$)]{\includegraphics[width=.7\textwidth]{RelResLocalModesL1InvGamZoom}}\\
\subfloat[][$\ell_{2,1}$ with gamma hyperprior ($SSR = 1$)]{\includegraphics[width=.7\textwidth]{RelResLocalModesL1GamZoom}}
\caption{A zoom into the plots in \Cref{fig:RelResChains}
\label{fig:RelResChainsZoom}}
\end{figure}



\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L22iGam_MAP_BestRelRes_XY}}
\hfill
\subfloat[][XY view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L22iGam_MAP_BestRelRes_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L22iGam_MAP_BestRelRes_XZ}}
\caption{MAP estimate with the best relative residuum (0.030) for $\ell_{2,2}$ hypermodel with inverse gamma hyperprior (red cones) and references sources (green cones).
\label{fig:L22InvGamMAPbRR}}
\end{figure}


\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21iGam_MAP_BestRelRes_XY}}
\hfill
\subfloat[][XY view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21iGam_MAP_BestRelRes_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21iGam_MAP_BestRelRes_XZ}}
\caption{MAP estimate with the best relative residuum (0.028) for $\ell_{2,1}$ hypermodel with inverse gamma hyperprior (red cones) and references sources (green cones).
\label{fig:L21InvGamMAPbRR}}
\end{figure}



\begin{figure}[tb]
\centering
\subfloat[][XY view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21Gam_MAP_BestRelRes_XY}}
\hfill
\subfloat[][XY view, zoom]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21Gam_MAP_BestRelRes_XY_zoom}}
\hfill
\subfloat[][XZ view]{\includegraphics[height=0.32\textwidth]{LpHyperModelsMEG_s12_L21Gam_MAP_BestRelRes_XZ}}
\caption{MAP estimate with the best relative residuum (0.066) for $\ell_{2,1}$ hypermodel with gamma hyperprior (red cones) and references sources (green cones).
\label{fig:L21GamMAPbRR}}
\end{figure}
